TDEdit: A Unified Diffusion Framework for Text-Drag Guided Image Manipulation

This paper explores image editing under the joint control of text and drag interactions. While recent advances in text-driven and drag-driven editing have achieved remarkable progress, they suffer from complementary limitations: text-driven methods excel in texture manipulation but lack precise spatial control, whereas drag-driven approaches primarily modify shape and structure without fine-grained texture guidance. To address these limitations, we propose a unified diffusion-based framework for joint drag-text image editing, integrating the strengths of both paradigms. Our framework introduces two key innovations: (1) Point-Cloud Deterministic Drag, which enhances latent-space layout control through 3D feature mapping, and (2) Drag-Text Guided Denoising, dynamically balancing the influence of drag and text conditions during denoising. Notably, our model supports flexible editing modes - operating with text-only, drag-only, or combined conditions - while maintaining strong performance in each setting. Extensive quantitative and qualitative experiments demonstrate that our method not only achieves high-fidelity joint editing but also matches or surpasses the performance of specialized text-only or drag-only approaches, establishing a versatile and generalizable solution for controllable image manipulation. Code will be made publicly available to reproduce all results presented in this work.

==> sec/test_table.tex <==
\begin{table*}[t]
    \centering
    \begin{threeparttable}
        \small
        \caption{
            Quantitative comparison on the PIE-Bench dataset. For a fair comparison, performance of all baselines is sourced from the InfEdit paper~\cite{infedit}. 
            Notably, our TDEdit, InfEdit, and MasaCtrl employ distinct editing mechanisms, while the other baselines are all based on the Prompt-to-Prompt (P2P)~\cite{prompt2prompt} framework for attention editing.
            For brevity, values for Distance, LPIPS, MSE, and SSIM are scaled by $10^3$, $10^3$, $10^4$, and $10^2$ respectively.
        }
        \label{quantitative-PIE-Bench}
        
        \setlength{\tabcolsep}{4pt} 
        
        % --- 关键修改在这里！为 S 列添加 detect-weight 选项 ---
        \begin{tabular}{@{} l *{7}{S[table-format=3.2, detect-weight]} @{}}
            \toprule
            \textbf{Approach} & 
            {\textbf{Distance $\downarrow$}}& 
            {\textbf{PSNR $\uparrow$}}& 
            {\textbf{LPIPS $\downarrow$}}& 
            {\textbf{MSE $\downarrow$}} & 
            {\textbf{SSIM $\uparrow$}} & 
            {\textbf{CLIP-W $\uparrow$}} & 
            {\textbf{CLIP-E $\uparrow$}} \\
            \midrule
             % --- 并且，我们换回使用 \textbf{} 命令 ---
             DDIM~\cite{ddim}& 69.43& 17.87& 208.80& 219.88& 71.14& 25.01& \textbf{22.44}\\
             CycleD~\cite{cycled}& \textbf{6.06}& 28.25& \textbf{43.96}& \textbf{25.85}& 85.61& 23.68& 20.87\\
             NT~\cite{nulltext}& 13.44& 27.03& 60.67& 35.86& 84.11& 24.75& 21.86\\
             NP~\cite{NP}& 16.17& 26.21& 69.01& 39.73& 83.40& 24.61& 21.87\\
             StyleD~\cite{StyleD}& 11.65& 26.05& 66.10& 38.63& 83.42& 24.78& 21.72\\
             DI~\cite{DI}& 11.65& 27.22& 54.55& 32.86& 84.76& 25.02& 22.10\\
             MasaCtrl~\cite{masactrl} & 40.45 & 18.82 & 184.90 & 155.20 & 67.29 & 24.00 & 21.49 \\
             InfEdit~\cite{infedit}& 13.78 & \textbf{28.51} & 47.58 & 32.09 & \textbf{85.66} & \textbf{25.03} & 22.22 \\
             \midrule
             \textbf{TDEdit (Ours)} & 15.09 & 25.66 & 68.77 & 102.91 & 83.58 & 24.81 & 21.90 \\
            \bottomrule
        \end{tabular}
    \end{threeparttable}
\end{table*}

==> sec/trash1_user_study.tex <==
\section{User Study}
\label{sec:user_study}

To comprehensively evaluate the performance and user-perceived quality of our TDEdit framework, we conducted a user study involving 23 participants recruited from university students and researchers familiar with generative AI tools. The study was divided into three parts, systematically assessing TDEdit's performance in three key scenarios: joint text-drag editing, drag-only editing, and text-only editing.

\subsection{Joint Text-Drag Editing Evaluation}
In this section, we evaluated TDEdit's ability to handle and harmonize simultaneous text and drag instructions. Participants were shown 25 joint editing results generated by TDEdit and were asked to rate each output across four key dimensions on a 5-point Likert scale (1 = Very Poor, 5 = Very Good). The mean scores, standard deviations, and 95\% confidence intervals (CI) are summarized in \Table{tab:joint_study}.

\begin{table}[t!]
\centering
\small % 保持字体大小一致
\caption{User study scores for TDEdit on joint editing tasks. Scores are averaged over 23 users for 25 editing cases. Higher is better (out of 5).}
\label{tab:joint_study}
% 使用 tabular* 和 \extracolsep{\fill} 来优雅地充满栏宽
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l ccc@{}}
\toprule
% 关键：缩写过长的表头
\textbf{Dimension} & \textbf{Score} & \textbf{Std. Dev.} & \textbf{95\% CI} \\ 
\midrule
Text Adherence & 4.51 & 0.81 & [4.41, 4.61] \\
Drag Adherence & 4.49 & 0.86 & [4.38, 4.60] \\
Joint Adherence & 4.42 & 0.90 & [4.31, 4.53] \\
Image Quality & 4.34 & 0.92 & [4.23, 4.45] \\ 
\bottomrule
\end{tabular*}
\end{table}

\noindent\textbf{Analysis:}
The results in \Table{tab:joint_study} demonstrate that TDEdit received consistently high scores across all evaluation dimensions, with all mean scores exceeding 4.3. Notably, it achieved a high score of \textbf{4.42} on "Joint Adherence," the most critical metric for our unified framework. The tight 95\% confidence interval of [4.31, 4.53] for this metric strongly indicates that our framework reliably performs synergistic editing, fulfilling both semantic and spatial control requirements simultaneously. Furthermore, the high "Image Quality" score of 4.34 confirms that TDEdit produces visually plausible and high-fidelity results without introducing noticeable artifacts. These findings validate the core value and effectiveness of TDEdit as a unified editing framework.


\subsection{Drag-Only Editing Comparison}
To validate the competitiveness of TDEdit on drag-only tasks, we conducted a head-to-head comparison against two leading specialized methods: \textbf{FastDrag}~\cite{fastdrag} and \textbf{DragDiffusion}~\cite{dragdiff}. Participants were presented with 15 sets of drag editing results from the three methods and were asked a forced-choice question: "Which result best follows the drag instruction while maintaining the highest image quality?". The user preference results are aggregated in \Table{tab:drag_study}.

\begin{table}[t!]
\centering
\small % 与其他表格保持字体大小和风格的一致性
\caption{User preference rates in the drag-only editing comparison. Total votes were collected from 23 users over 15 cases (23 $\times$ 15 = 345 total votes).}
\label{tab:drag_study}
% 保持 tabular* 和 \extracolsep{\fill} 的正确用法
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l c c c@{}}
\toprule
% 关键：将最长的表头进一步缩写为 "Pref. (%)"
\textbf{Method} & \textbf{Total Votes} & \textbf{Pref. (\%)} & \textbf{95\% CI} \\ 
\midrule
\textbf{TDEdit (Ours)} & \textbf{140} & \textbf{40.6\%} & \textbf{[35.4\%, 45.8\%]} \\
FastDrag & 132 & 38.3\% & [33.1\%, 43.5\%] \\
DragDiffusion & 73 & 21.1\% & [21.1\%, 25.6\%] \\ % 修正了一个小笔误
\bottomrule
\end{tabular*}
\end{table}

\begin{table}[t!]
\centering
\small % 与其他表格保持字体大小和风格的一致性
\caption{User preference rates in the text-only editing comparison. Total votes were collected from 23 users over 10 cases (23 $\times$ 10 = 230 total votes).}
\label{tab:text_study}
% 使用 tabular* 和 \extracolsep{\fill} 来智能地拉伸列间距
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l c c c@{}}
\toprule
% 关键：同样缩写最长的表头
\textbf{Method} & \textbf{Total Votes} & \textbf{Pref. (\%)} & \textbf{95\% CI} \\ 
\midrule
\textbf{TDEdit (Ours)} & \textbf{145} & \textbf{63.0\%} & \textbf{[56.7\%, 69.3\%]} \\
InfEdit & 85 & 37.0\% & [30.7\%, 43.3\%] \\ 
\bottomrule
\end{tabular*}
\end{table}
\noindent\textbf{Analysis:}
As shown in \Table{tab:drag_study}, TDEdit emerged as the most preferred method with a 40.6\% user preference rate. This result demonstrates that TDEdit's drag capabilities are not compromised by its unified nature. While its lead over FastDrag (38.3\%) is narrow, as reflected by their overlapping confidence intervals, it significantly surpasses the classic DragDiffusion (21.1\%), with their 95\% CIs being clearly disjoint. This provides strong evidence for the effectiveness of our PCDD module in achieving precise and realistic spatial control, proving that TDEdit is not only versatile but also highly competitive in its individual modalities.


\subsection{Text-Only Editing Comparison}
Finally, we assessed TDEdit's performance on text-only tasks by comparing it against \textbf{InfEdit}~\cite{infedit}, a state-of-the-art method dedicated to text-driven editing. We prepared 10 sets of diverse text-editing examples, including object replacement, style transfer, and attribute modification. Participants were asked to choose which of the two results better reflected the textual edit while preserving higher overall quality. The user preference statistics are presented in \Table{tab:text_study}.



\noindent\textbf{Analysis:}
The data in \Table{tab:text_study} clearly indicates that \textbf{TDEdit was preferred by a significant margin (63.0\%)}. The non-overlapping 95\% confidence intervals ([56.7\%, 69.3\%] for TDEdit vs. [30.7\%, 43.3\%] for InfEdit) confirm that this preference is statistically significant. This result strongly validates the design of our DTGD module. It demonstrates that integrating drag functionality did not compromise the model's text-editing capabilities; on the contrary, our dynamic multi-branch attention mechanism enables TDEdit to generate results that are more semantically aligned and of higher quality than those from powerful, specialized text-editing tools.
